Riemannian Direct Trajectory Optimization of Rigid Bodies on Matrix Lie Groups

Designing dynamically feasible trajectories for rigid bodies is a fundamental problem in robotics. Although direct trajectory optimization is widely applied to solve this problem, inappropriate parameterizations of rigid body dynamics often result in slow convergence and violations of the intrinsic topological structure of the rotation group. This paper introduces a Riemannian optimization framework for direct trajectory optimization of rigid bodies. We first use the Lie Group Variational Integrator to formulate the discrete rigid body dynamics on matrix Lie groups. We then derive the closed-form first- and second-order Riemannian derivatives of the dynamics. Finally, this work applies a line-search Riemannian Interior Point Method (RIPM) to perform trajectory optimization with general nonlinear constraints. As the optimization is performed on matrix Lie groups, it is correct-by-construction to respect the topological structure of the rotation group and be free of singularities. The paper demonstrates that both the derivative evaluations and Newton steps required to solve the RIPM exhibit linear complexity with respect to the planning horizon and system degrees of freedom. Simulation results illustrate that the proposed method is faster than conventional methods by an order of magnitude in challenging robotics tasks.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> logic.tex <==
\section{Logic}
\harry{LC comments to be addressed...}
\begin{enumerate}
    \item Problem statement: filtering of polynomial dynamical systems
    \item Polynomial KF: procedural presentation of propagation and update, and give some intuition about why they make sense and the fact that there is no longer a closed-form solution but we need to solve optimization problems.
    \item For r=1 and Gaussian noise this becomes KF
    \item Show why it makes sense, in particular: (i) BPUE vs BLUE, (ii) why covariance can be "approximately" extracted from the dual, (iii) show marginalization for the propagation step.
    
\end{enumerate}
Furthermore, we provide both quantitative and qualitative results that demonstrate the effectiveness of our proposed filtering technique on highly nonlinear dynamical systems with highly non-Gaussian noises. 
\harry{Look for missing Experiments}:
\begin{enumerate}
    \item prediction: show that after prediction GKF produces a banana-shaped distribution, while EKF produces a less accurate distribution (see this for inspiration: https://www.roboticsproceedings.org/rss08/p34.pdf)
    \item update step: BPUE ablation: linear case, binary/non-gaussian noise, evaluation of covariances (and show they empirically make sense)
    \item do just a localization experiment comparing with EKF and using a very nonlinear measurement model, e.g., range only or range/bearing + motion in SE(2). some serious ablation on noise magnitude. Maybe use Victoria Park but with fixed landmarks: \url{https://www.mrpt.org/Dataset_The_Victoria_Park} (or a 2D localization dataset? google: "landmark-based 2D localization"). 
\end{enumerate}

\begin{equation}
     T_k^{-1}X_k^{-1}X_{k+1} = w_k
\end{equation}
% \begin{abstract}

% \end{abstract} 

% \IEEEpeerreviewmaketitle
% \begin{enumerate}[1.]
%     \item Define the BPUE as a optimization on rank-one ``moment'' matrix, thus we have the notion of tangent space and the covariance in the tangent space.
%     \item Solve the BPUE using SDP relaxation. Show the generalized Kalman gain. Then we have the update of the covariance at the limiting case (at the same tangent space). % \tsl{The vector transport? } 
%     \item Once we have the covariance defined in tangent space, we can marginalize by extracting the sub-principle matrix of the rank-one moment matrix. 
% \end{enumerate}
\tsl{TODO: About the presentation. }
\begin{enumerate}
    \item Define BPUE as BLUE plus QCQP moment matrix constraints.
    \item Solve the BPUE using SDP relaxation. Show the generalized Kalman gain. Then we have the update of the covariance at the limiting case (at the same tangent space). % \tsl{The vector transport? } 
    \item Once we have the covariance defined in tangent space, we can marginalize by extracting the sub-principle matrix of the rank-one moment matrix. 
\end{enumerate}


==> text_v3/GMKF.tex <==
\section{\GMKFlong}

In this section, we introduce \GMKF. We predict the moments in the propagation steps leveraging the system dynamics and recover the distribution. In the update steps, we formulate the observation model as another max entropy distribution and renew the parameters.

\subsection{Extended Dynamical System }
% \tsl{Actually we only use the extended observation}
To utilize the higher-order moments of the noise, we need an extended version of system \eqref{eq:polyDynSys} that exposes the moments of the noise in the state-space model.
%includes the higher-order terms of noise in the state space model.
% \begin{definition}[Extended polynomial dynamical system] 
% $\M \phi_r(\cdot)$ 
To achieve this goal, we apply $\vv_r(\cdot)$ to both sides of eq.~\eqref{eq:polyDynSys} to generate monomials of degree up to $r$ from the entries of $\M w_k$ and $\M v_k$: 
\tsl{I am replacing $\phi$ with $v$ to have a homogeneous equation that cause less trouble in computation and definition of system.}
\begin{equation}
\begin{aligned}
    \label{eq:ext-polyDynSys}
    &\left\{
	\begin{array}{l}
	\vv_r\left(\M x_{k+1} \right) = \vv_r(\M f(\M x_{k}, \M u_k, \M w_k )) \\
	\vv_r\left(\M h( \M y_k, \M x_{k} )\right) = \vv_r(\M v_k) \\
	\end{array}.
\right. \\
\end{aligned}
\end{equation}
Intuitively, eq.~\eqref{eq:ext-polyDynSys} combines the entries of the original process and measurement models into higher-order polynomials by taking powers and products of the entries of $\M f$ and $\M h$. Below, we refer to $\vv_r(\M w_k)$ and $\vv_r(\M v_k)$ as the \emph{extended noise}.  % and $r$ as the \emph{extended degree}}.

Since each polynomial of degree up to $r$ can be written as a linear combination of the monomial basis $\vv_r(\M{x}), $\footnote{The non-expert reader can find examples in Appendix~\ref{appx:momcond_linear}.}
we can rewrite both the extended dynamics or the dynamics as linear expressions of the monomials in $\M{\phi}_r(\M{x})$:
\begin{equation}
\label{eq:bs-ext}
\left\{
	\begin{array}{l}
    \vv_r(\M x_{k+1}) = \M A(\M w_k, \M u_k) \vv_s(\M x_{k}) \\ %  + \M b(\M w_k, \M u_k) \\
    \M{C}(\M{y}_k)\vv_q(\M{x})  = \vv_r(\M{v}_k) %  + \M{d}(\M{y}_k)
    \end{array}\right.
\end{equation}
Note that as the the $\vv_s(\M x_{k})$ on the RHS of the dynamics may have different degree as LHS due to the nonlinearity, thus we have the order possibly $r\neq s, r\neq q$. We also note that the first term of $\vv_r(\cdot)$ is always $1$ that enable us to define the dynamics as a homogeneous linear equality of the monomials.


\subsection{Initialization}
We provide the initial state as a maximal entropy distribution with initial coefficients $\M \lambda^+_0$
\begin{equation}
    p(\M x|\M \lambda^+_0) = \exp{\left(-\sum_{\alpha}\lambda^+_{0, \alpha} \M x^{\alpha} \right)}.
\end{equation}
One typical choice is the Gaussian distribution, which is a max entropy distribution with constraints on the mean and covariance. The corresponding moments $\bar{\M x}_{\alpha}$ can be obtained via numerical integration, for general cases.

\subsection{Propagation Steps}
% In the propagation steps, we leverage the dynamics of the system to predict the moments of the next time step and recover the distribution via \Cref{alg:trust-lambda}. 
Consider the extended dynamics:
\begin{equation}
\label{eq:ext-dyn}
    \vv_r(\M x_{k+1}) = \M A(\M w_k, \M u_k) \vv_s(\M x_{k}). % + \M b(\M w_k, \M u_k). 
\end{equation}
The moments of belief $p(\M x_{k+1})$ can be obtained via taking expectation on both side of \eqref{eq:ext-dyn}. Thus we have:
\begin{equation}
    \mathbb{E}[\vv_r(\M x_{k+1})] = \mathbb{E}[\M A(\M w_k, \M u_k) \vv_s(\M x_{k})]. %  + \M b(\M w_k, \M u_k)
\end{equation}
Under the assumption that the the noise distribution is independent with the state distribution, the above equation can be simplified by the following linear equations on the moments:
\begin{equation}
    \bar{\M x}_{\alpha,k+1} = \M A(\bar{\M w}_{\gamma}, {\M u}_k) \bar{\M x}_{\beta,k}, % + \M b(\bar{\M w}_{\gamma}, \M u_k)
\end{equation}
with the dimension specified by $\alpha \in \mathbb{N}_r^n, \beta \in \mathbb{N}_s^n$.
Given the moments sequence $\bar{\M x}_{\alpha,k+1}$, we can apply \Cref{alg:tro-hierarchical} to recover the distribution represented by $\M \lambda^-_{k+1}$, i.e.,
\begin{equation}
    p(\M x_{k+1} | \M\lambda^-_{k+1}). 
\end{equation}

\subsection{Update Steps}
In the update steps, we consider to formulate the sensor model as a max entropy distribution. Consider the extended measurement model:
\begin{equation}
    \M{C}(\M{y})\vv_q(\M{x}) = \vv_r(\M{v}). % + \M{d}(\M{y}) 
\end{equation}
Given the moments of $\M\phi_r(\M{v})$, i.e., $\bar{\M v}_{\alpha}$, we have the max entropy distribution of the noise via \Cref{alg:tro-hierarchical}, parameterized by $\M \mu$
\begin{equation}
    p(\M v) = \exp{\left(-\sum_\alpha \mu_{\alpha} \M v^{\alpha} \right)}.
\end{equation}
As the value of $\M v$ is related to the state $\M x$ by the observation model:
\begin{equation}
    \M v = \M h(\M y, \M x),
\end{equation}
the distribution of the $\M y$ under measurement $\M x$ can be obtained via substitution of the observation model. Thus, we have the likelihood function:
\begin{equation}
\label{eq:obs-model}
\begin{aligned}
    p_{\M \mu}(\M x | \M y ) &= \exp{\left(-\sum_\alpha \mu_{\alpha} \M h(\M y, \M x)^{\alpha} \right)} \\
    &=\exp{\left(-\sum_\alpha \nu_{\alpha} \M x^{\alpha} \right)}
\end{aligned}
\end{equation}
With a batch of $m$ measurements, and the prior distribution $p(\M x | \M \lambda^-)$, the distribution of $\M x$ can be obtained via:
\begin{equation}
\begin{aligned}
    p(\M x | \M\lambda^+) \propto p(\M x | \M \lambda^{-}) \prod_{i=1}^m p_{\M \mu}(\M x | \M y_i) = \exp{\left( -\sum_\alpha \lambda_{\alpha}^{+}\M x^{\alpha}  \right) }.
\end{aligned}
\end{equation}
with $\M \lambda^+$ being the summation of the coefficients:
\begin{equation}
\label{eq:update-lambda}
    \M \lambda^+ = \M \lambda^- + \sum_i^m \M\nu_i.
\end{equation}
Normalization is only needed when computing the moments for belief propagation.
% To compute the moments of $p(\M x | \M\lambda^+)$, we apply numerical integration over the domain of $\mathcal{K}$. 

\subsection{Extraction of Optimal Point Estimation}

\begin{algorithm}[t]
\label{alg:general}

\caption{\GMKFlong}\label{alg:gmkf}

\begin{algorithmic}
\footnotesize
\Require Initial distribution parameterized by $\M \lambda^+_0$, dynamics model $\M x_{k+1} = \M f(\M x_k, \M u_k, \M w_k)$, observation model $\M h(\M y, \M x) = \M v$. \\

\State {\texttt{// Obtain the observation model}} 
\State $ \M \mu_{\beta} \xleftarrow{\mathrm{Alg. \ref{alg:tro-hierarchical}}} \bar{\M v}_{\beta}  $\\

\For{time $k = 1, \ldots, N$}
    \tsl{Add two ifelse to indicate if the measurement are obtained. }
    \State {\texttt{// Compute the moments at $k-1$}}
    \State $\M x_{\beta, k-1} \gets \int_{\mathcal{K}} p(\M x | \M\lambda^+_{k-1})\M x^{\beta}d\M x  $ \\
    \State {\texttt{// Propagation of moments via dynamics}}
    \State $\bar{\M x}_{\alpha,k} \gets \M A(\bar{\M w}_{\alpha}, {\M u}_{k-1}) \bar{\M x}_{\beta,k-1} + \M b(\bar{\M w}_{\alpha}, \M u_{k-1})$ \\
    \State \tsl{Quotient ring reconstruction has numerical issues, we can construct Gaussian belief in prediction instead as a temporary solution.}

    \tsl{Need to consider rescaling of the variable. The Dirac measure is super hard for integration.}
    
    \State {\texttt{// Reconstruct the distribution}}
    \State $ \M\lambda^-_{k} \xleftarrow{\mathrm{Alg. \ref{alg:trust-lambda}}} \bar{\M x}_{\alpha,k}  $
    \\

    \State {\texttt{// Update with measurements} }
    \State $\M \nu_k \xleftarrow{\eqref{eq:obs-model}} \M y_k, \M \mu_{\beta} \quad \M\lambda^+_{k} \gets \M\lambda^-_k + \M \nu_k $ \\

    \State {\texttt{// Normalize the distribution}}
    \State $\lambda^+_{k, \alpha_0} \gets \lambda^+_{k, \alpha_0} - \ln{\int_{\mathcal{K}}p(\M x | \M \lambda^+_k) d\M x } $ \\

    \State {\texttt{// Extract the optimal point estimation}}
    \State $\M x_k^*, \M X^*_k \xleftarrow{\mathrm{\eqref{prob:pop_sdp}}} \min_{\M x \in \mathcal{K}}  -\ln{p(\M x | \M\lambda_k^+)}$
    \tsl{Mention the rounding algorithm here.}
\EndFor \\
\end{algorithmic}
\end{algorithm}


As the \GMKF provides the belief representation with higher-order moments, it is not straightforward to obtain the point estimation in the sense of maximal likelihood as in Gaussian case. Consider the getting the optimal point estimation via
\begin{equation}
\label{eq:point-estimation}
    \max_{\M x \in \mathcal{K}}\ \ p(\M x|\M\lambda) \Leftrightarrow \min_{\M x \in \mathcal{K}}\ \ -\ln{p(\M x | \M\lambda)}. 
\end{equation}
As we only have moment constraints, \eqref{eq:point-estimation} is a \eqref{prob:pop} with the polynomial cost function being the negative log-likelihood:
\begin{equation}
\begin{aligned}
    \min_{\M x} \quad &\sum_\alpha \lambda_{\alpha} \M x^{\alpha}\\
    \mathrm{s.t. }\quad & \M x \in \mathcal{K}
\end{aligned}.
\end{equation}
Thus, we instead solve \eqref{prob:pop_sdp} to extract the optimal point estimation that have the highest density. Under the condition that \eqref{prob:pop_sdp} has rank-1 solution, the optimal point estimation can be extracted and certified by the rank condition. In the case that the optimization does not have rank-1 solution, a rounding algorithm is presented in appendix XX using gradient based local solvers.
Finally, we summarize the \GMKF in \Cref{alg:gmkf}. 



==> text_v3/GeodesicBasedCostFunction.tex <==
\section{Geodesic Based Cost Function Design}
In this section, we introduce the geodesic-based cost function design. 

\subsection{Riemannian Hessian in Coordinates}
Consider a cost function:
\begin{equation}
    f(x): \mathcal{M} \rightarrow \mathbb{R}
\end{equation}
with the gradients $\operatorname{grad} f$. To derive the Hessian via the Riemannian connection, we first express the gradients in local coordinates $\phi$ in terms of the vector field $\left\{E_1, E_2, \cdots, E_n\right\}$:
\begin{equation}
    \operatorname{grad} f = \sum_i h_i(\phi) E_i 
\end{equation}
Remember the axiomatic definition of Hessian, we consider $u \in \operatorname{T}_x\mathcal{M}$ expressed in coordinates:
\begin{equation}
    u = \sum_i u_i E_i.
\end{equation}
Then we proceed to derive the Hessian via:% \mgj{we should introduce Einstein summation notation and drop the summation. Then $\sum_i u_i E_i = u^i E_i$. The diff geom notation uses lower and upper indices for coordinates and basis. Will can double check to make sure they're correct. Add Will to the overleaf when it's readable. This version is more readable for engineers though.}\tsl{I will add Will later! This version is what I actually coded in MATLAB.}
\begin{equation}
\begin{aligned}
    \operatorname{Hess} f[u] &= \nabla_{u} \operatorname{grad} f \\
                          &= \nabla_{\sum_i u_i E_i } \sum_j h_j(\phi) E_j  \\
                          & \quad \quad \text{Linearity w.r.t $u$ and $\operatorname{grad} f$ } \\
                          &= \sum_i u_i \left(\nabla_{E_i } \sum_j h_j(\phi) E_j\right)  \\
                          & \quad \quad \text{Leibniz rule} \\
                          &= \sum_i u_i \left(  \sum_j  \operatorname{D}h_j(\phi)[E_i] E_j +  h_j(\phi) \nabla_{E_i }E_j\right)  \\
\end{aligned}
\end{equation}
which is linearly dependent on $u$. 

\subsection{Geodesic on $\mathrm{SO}(3)$ }

Consider a cost function:
\begin{equation}
    f(\log{(X)}): \mathcal{G} \rightarrow \mathbb{R}
\end{equation}
the cost function can be obtained via:
\begin{equation}
   \operatorname{grad} f = \frac{\partial f(\phi)}{\partial \phi}\frac{\partial \log{(X)} } {\partial X}, \phi = \log{X}
\end{equation}
In the $\mathrm{SO}(3)$ case, the Jacobians of $\log{(X)}$ has closed form solutions parameterized by $\phi$. Namely, we have 
\begin{equation}
    \operatorname{grad} f = \sum_i h_i(\phi) E_i 
\end{equation}
Then we proceed to derive the Hessian via:
\begin{equation}
\begin{aligned}
    \operatorname{Hess} f &= \nabla_{u} \operatorname{grad} f \\
                          &= \nabla_{\sum_i u_i E_i } \sum_j h_j(\phi) E_j  \\
                          &= \sum_i u_i \left(\nabla_{E_i } \sum_j h_j(\phi) E_j\right)  \\
                          &= \sum_i u_i \left(\nabla_{E_i } \sum_j h_j(\phi) E_j\right)  \\
                          &= \sum_i u_i \left(  \sum_j  \operatorname{D}h_j(\phi)[E_i] E_j +  h_j(\phi) \nabla_{E_i }E_j\right)  \\
\end{aligned}
\end{equation}


% \subsection{Geodesics on Matrix Lie Group $\mathrm{SO(3)}$ }
% \begin{equation}
    
% \end{equation}


==> text_v3/Numerical.tex <==
\section{Numerical Experiments}
In this section, we verify \GMKF in a few examples. 

\subsection{Asymptotic Property of Max Entropy Distribution}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/asymptotic.pdf}
    \caption{The max entropy distribution with moment matched up to order $r$. The heat map and samples are shown on the RHS of the plots. WE observe that as the order increase, the approximated distribution asymptotically approach the sampled distribution. }
    \label{fig:asymptotic}
\end{figure*}

We first showcase the asymptotic property of max entropy distribution and verify the correctness of \Cref{alg:trust-lambda} and \ref{alg:tro-hierarchical}. 

We consider a distribution:
\begin{equation}
\label{eq:trig-noise}
    \M v = \begin{bmatrix}
        \sin{w} + \epsilon_1\\
        \cos{\pi w} + \epsilon_1
    \end{bmatrix} + \M \epsilon
\end{equation}
where $w\sim U(0, \pi)$ is a uniform distribution between $0$ and $\pi$, and $\epsilon_1, \epsilon_ 2\sim \mathcal{N}(0, 0.01)$ is a Gaussian noise. We draw $N=1e5$ samples from the distribution to compute mean values an unbiased estimation of the underlying moments, i.e, 
\begin{equation}
    \hat{\M v}_{\alpha} =  \frac{1}{N} \sum^N_{k=1}\M v_{k}^\alpha, \alpha \in \mathbb{N}^n_r.
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=1 \columnwidth]{figures/trust-region-convergence.pdf}
    \caption{The convergence of each optimization with moments up to $r$ are matched. Quadratic convergence rate is observed due to the Newton steps. }
    \label{fig:convergence}
\end{figure}

The samples and max entropy distribution with moment up to order $r$ are shown in \Cref{fig:asymptotic}. We observe that as more moments are matched, the distribution asymptotically approach the sampled distribution. The result is expected according to \Cref{theorem:asymptotic}. When $r = 2$, the max entropy is the Gaussian distribution. Due to the nonlinear transformation, the samples are concentrated around the location on the curve with larger curvature, which are clearly indicated by the $p(\M x | \M \lambda)$ when $r \ge 4$. The norm of the gradients in each optimization is illustrated in \Cref{fig:convergence}. Quadratic convergence, a sign of second-order optimization, is observed to demonstrated the success of the algorithm \Cref{alg:trust-lambda}. \ref{alg:tro-hierarchical} terminates at $r=12$ and we can verify that the result of $r=12$ is sufficiently good by comparing it with the heat map of the samples. 


\subsection{Update Steps}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/update-recursive.pdf}
    \caption{The convergence of each optimization with moments up to $r$ are matched. Quadratic convergence rate is observed due to the Newton steps. }
    \label{fig:update-recursive}
\end{figure*}


Now we verify the update steps \GMKF. We consider a basic linear observation:
\begin{equation}
    \M y = \M x + \M v \in \mathbb{R}^2. 
\end{equation}
where the moment of $\M v$ is known in advance. Then we consider the nonlinear noise in last section and a discrete noise:
\begin{equation}
\label{eq:bin-noise}
    \M v = \begin{bmatrix}
        2q_1 - 1 + \epsilon_1 \\
        2q_2 - 1 + \epsilon_2
    \end{bmatrix}
\end{equation}
where $q_1, q_2 \sim \mathrm{Bernoulli(0.5)}$ and $\epsilon_1, \epsilon_2 \sim \mathcal{N}(0, 0.2\M I)$. \Cref{alg:tro-single} terminates at $r=2$ for this discrete noise. 

We compare the proposed method with the Best Linear Unbiased Estimator, which is the minimal variance estimator using only mean and covariance. 
We compare the asymptotic property of the update steps with accumulated measurements. We accumulate $N$ measurements to obtain the negative log-likelihood, i.e, 
\begin{equation}
    -\ln{p(\M x | \M y_1, \M y_2, \cdots, \M y_N)} = \mathrm{Scalar} + \sum_{k=1}^N \sum_{\alpha} \mu_{\alpha} \M h(\M y_k, \M x)^{\alpha}.
\end{equation}
The normalized belief distribution for the case with binary noise is illustrated in \Cref{fig:update-recursive}. We notice that after receiving the first measurement, the belief computed by $r=2$ keeps the multi-modality caused by the noise distribution to indicate four mostly possible locations. After more measurements are incorporated, the belief converges to the true state with dramatically smaller covariance. The result with noise \eqref{eq:trig-noise} are shown in \Cref{fig:update-trig}, which exhibit similar patterns. 

We further sample $1000$ trials in each noise with different $N$ to compute the empirical variance of the point estimation. The result are presented in \Cref{table:cov_trig} and \ref{table:cov_bin}. We observe that with sufficiently many measurements accumulated ($N\ge5$), increasing $r$ consistently lowers the covariance and outperform BLUE dramatically. With small $N$, the multi-modality of the belief introduces additional bias when computing the point estimation that make the covariance higher than BLUE. However, we note that the point estimation is not a full belief representation and can not represent the multi-modality. 

\begin{table}%[b]
\setlength\tabcolsep{2.5pt}
\centering
% \small
\tiny
% \scriptsize
\caption{Covariance of rank-1 point estimation with $N$ accumulated samples using noise model \eqref{eq:trig-noise} with moments up to order $r$ matched.}
\begin{tabular}{c|cccccccc}
\hline
$N$ &  $1$& $2$ & $3$ & $5$ & $10$  & $20$ & $50$ & $100$ \\ \hline
$r=2$ &  $1.583$& $0.805$ & $5.39e^{-1}$ & $3.26e^{-1}$ & $1.63e^{-1}$  & $7.84e^{-2}$ & $3.19e^{-2}$ & $1.61e^{-2}$   \\
$r=4$ &  $3.379$& $1.581$ & $7.71e^{-1}$ & $1.87e^{-1}$ & $3.03e^{-2}$  & $1.014e^{-2}$ & $3.470e^{-3}$ & $1.71e^{-3}$  \\
$r=6$ &  $4.482$& $1.800$ & $6.96e^{-1}$ & $1.59e^{-1}$ & $2.10e^{-2}$  & $3.54e^{-3}$ & $8.94e^{-4}$ & $4.27e^{-4}$ \\
$r=6$ &  $4.521$& $1.825$ & $6.61e^{-1}$ & $1.31e^{-1}$ & $7.09e^{-3}$  & $9.30e^{-4}$ & $2.72e^{-4}$ & $1.34e^{-4}$ \\
$r=10$ & $4.044$& $1.829$ & $6.28e^{-1}$ & $5.96e^{-2}$ & $1.06e^{-3}$  & $3.078e^{-4}$ & $1.07e^{-4}$ & $4.69e^{-5}$\\
$r=12$ &  $2.410$& $1.723$ & $3.67e^{-1}$ & $2.30e^{-2}$ & $3.78e^{-4}$  & $1.75e^{-4}$ & $7.12e^{-5}$ & $3.27e^{-5}$  \\ \hline
\end{tabular}
\label{table:cov_trig}
\end{table}

\begin{table}%[b]
\setlength\tabcolsep{2.5pt}
\centering
% \small
\tiny
% \scriptsize
\caption{Covariance of rank-1 point estimation with $N$ accumulated samples using noise model \eqref{eq:bin-noise} with moments up to order $r$ matched.}
\begin{tabular}{c|cccccccc}
\hline
$N$ &  $1$& $2$ & $3$ & $5$ & $10$  & $20$ & $50$ & $100$ \\ \hline
$r=2$ &  $2.073$& $1.009$ & $7.06e^{-1}$ & $4.20e^{-1}$ & $2.08e^{-1}$  & $9.89e^{-2}$ & $4.07e^{-2}$ & $1.99e^{-2}$   \\
$r=4$ &  $4.471$& $2.051$ & $1.141$ & $2.72e^{-1}$ & $1.28e^{-2}$  & $4.59e^{-3}$ & $1.90e^{-3}$ & $9.36e^{-4}$  \\ \hline
\end{tabular}
\label{table:cov_bin}
\end{table}

% trig
% 1.58290123502627	0.805310514145445	0.538533777966679	0.326179713582760	0.163348263760269	0.0784036692077170	0.0318534986581001	0.0160527682348476
% 3.37898475117888	1.58149355877769	0.771256282325694	0.187245834269611	0.0302623622856440	0.0101354464220757	0.00347024817212813	0.00171783188427215
% 4.48195239001133	1.79980006788561	0.696105500152692	0.159424717706419	0.0205094222357977	0.00354402864117936	0.000893538750196796	0.000426565934220236
% 4.52146465545775	1.82525451119380	0.660763204407800	0.130733886244268	0.00709430268960970	0.000925565569774268	0.000271710566606747	0.000134237241271038
% 4.04481119754960	1.82870477369091	0.627897938797634	0.0595938308082545	0.00105737721255847	0.000307819912426411	0.000107210410118413	4.69458523946517e-05
% 2.40827424246039	1.72290432449246	0.367302904338136	0.0230581999758475	0.000378088826805819	0.000175026552444545	7.12370142299247e-05	3.27491698898325e-05

% bin
% 2.07287363283234	1.00889145462304	0.705659358249660	0.420031906824069	0.208496401314326	0.0989109458412624	0.0407175589431104	0.0198907661793532
% 4.47085360077634	2.05054907175109	1.14104403501219	0.271743907272533	0.0128121311053057	0.00459255181448723	0.00189899882714455	0.000936220599647427

% \tsl{Explain the reason for the bias. This is a belief representation, thus the point estimation may not be proper.}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/update-trig.pdf}
    \caption{From the top to bottom, the use of noise distribution model with moment order $r = 2, 4, 6, 8, 10$ and $12$ are matched. As more measurements are incorporated, the belief converges to the true state. We notice that with larger $r$, the belief converges much faster to the Dirac measure. }
    \label{fig:update-trig}
\end{figure*}


\subsection{Localization with Unknown Data Association on $\mathrm{SE}(2)$ }
We consider the configuration of the robot on $\mathrm{SE}(2)$, i.e, 
\begin{equation}
    \M Z := \begin{bmatrix}
        c & -s & p_x \\
        s &  c & p_y \\
        0 & 0 & 1
    \end{bmatrix}, \M x:= \begin{bmatrix}
        c \\
        x \\
        p_x \\
        p_y
    \end{bmatrix},
\end{equation}
with one constraint:
\begin{equation}
    g(\M x) = c^2 + s^2 - 1 = 0.
\end{equation}
We also denote the rotation and the position separately:
\begin{equation}
    \M R:=\begin{bmatrix}
        c & -s \\
        s &  c \\
    \end{bmatrix}, \M p:=\begin{bmatrix}
        p_x \\
        p_y \\
    \end{bmatrix}.
\end{equation}
Finally the systems can be expressed as:
    \begin{equation}
    \label{eq:polyDynSys}
\left\{
	\begin{array}{l}
    \M Z_{k+1} = \M Z_k \M U_k \M W_k \in \mathrm{SE}(2) \\
    \M y = \M R^{\transpose}(\M p - \M p^L + \M v)
	\end{array}, 
\right.
\end{equation}
with the pose $\M Z$, input $\M U$, and noise $\M W$ all defined on $\mathrm{SE}(2)$. In the observation model, $\M p^L$ is the position of center of the landmarks and $\M v$ is a noise that models the unknown data association. The noise $\M W$ is assumed to generated by the differential wheel dynamics in \cite{long2013banana} in Lie algebra. Here we convert it to matrix Lie group.  

We first present the result with only prediction and compare with Monte Carlo simulation. 

\subsection{Lidar-based Localization}

==> text_v3/RIPM.tex <==
\subsection{Riemannian Interior Point Method}
\subsection{Newton's Iteration on Riemannian Manifold}

==> text_v3/RigidBodyDynamics-NullSpace.tex <==
\section{Discrete Rigid Body Dynamics}
\label{sec:formulation}
% We introduce the discrete rigid body dynamics induced by the variational integrators.
In this section, we derive the rigid body dynamics based on the variational integrators on $\mathcal{M}_{\mathrm{RB}}$. The polynomial structure of $\mathcal{M}_{\mathrm{RB}}$ is leveraged to eliminate the constraint forces by holonomic constraints. 

\subsection{Variation-based Discretization}
% Though directly integrate \eqref{eq:forcedEP} using conventional integrators such as Euler first-order integration provides discrete equation of motion, these methods do not preserve the energy and breaks the symmetry on matrix Lie groups. Instead, we consider the variation-based discretization that provides a symmetric EoM on matrix Lie group.

Consider a mechanical system with the configuration space $Q$. We denote the configuration state as $q \in Q$ and the generalized velocity as $\dot{q} \in T_{q}Q$. Then we have the Lagrangian given the kinetic and potential energy $T(\dot{q}), V(q)$:
\begin{equation}
\label{eq:ct_lag}
    L(q, \dot{q}):=T(\dot{q}) - V(q). 
\end{equation}
The key idea of a variational integrator is to discretize the Lagrangian \eqref{eq:ct_lag} to obtain the discrete-time EOM \cite{marsden2001discrete}. The discretization scheme ensures that the Lagrangian is conserved in discrete time, thus having superior energy conservation properties in the long duration. 
% We define the time step $h \in \mathbb{R}$ and the time sequence \mbox{$\{t_k = kh \mid  k = 0, \dots, N\} \subset \mathbb{R}$}. 
The discrete Lagrangian $L_d: Q\times Q \rightarrow \mathbb{R}$ could be considered as the approximation of the action integral via:
\begin{equation}
\label{eq:lag_ct2dt}
    L_d(q_k, q_{k+1}) \approx \int ^{t_{k+1}}_{t_k}L(q, \dot{q})dt .
\end{equation}
% In this work, we consider the midpoint approximation \cite{marsden2001discrete}:
% \begin{equation}
% \label{eq:dt_lag_int}
%     L_d(q_k, q_{k+1}) = hT(\frac{q_{k+1} - q_k}{h}) - hV(\frac{q_{k+1} + q_k}{2}).
% \end{equation}
Then the discrete variant of the action integration becomes:
\begin{equation}
    S_d = \sum_{k=0}^{N-1}{L}_d(q_k, q_{k+1}) .
\end{equation}
% where $\bar{L}_d(q_k, q_{k+1})$ is the sum of the midpoint approximation defined in \eqref{eq:dt_lag_int} and \eqref{eq:dt_force_int}. 
Finally, we take variation in $TQ$ and group the term corresponding to $\delta q_{k} \in T_{q_k}Q$ as the discrete version of integration by parts \cite{marsden2001discrete}: 
\begin{equation}
\begin{aligned}
  \delta S_d &= \langle D_1 {L}_d(q_0, q_1), \delta q_0 \rangle +  \langle D_2 {L}_d(q_{N-1}, q_N),  \delta q_N \rangle\\ 
    &+ \sum_{k=1}^{N-1}
    \langle D_2 {L}_d(q_{k-1}, q_k) + D_1 {L}_d(q_k, q_{k+1}), \delta q_k \rangle. 
\end{aligned}
\end{equation}
where $D_i$ denotes the derivative with respect to the $i$-{th} argument and $\langle \cdot, \cdot\rangle$ the canonical inner product.  
By the least action principle, the stationary point can be determined by letting the derivative of $\delta q_k$ being zero: 
\begin{equation}
\label{eq:discrete_eom}
D_1L_d(q_k, q_{k+1}) + D_2L_d(q_{k-1}, q_{k}) = 0. % Bf_d(t_k)
\end{equation}

To consider the external force $u$ we consider the action integral of control input $u(t)$:
\begin{equation}
    \int_{t_k}^{t_{k+1}} \langle u(t), \delta q \rangle dt \approx \frac{\Delta t}{2} \langle u(t_k), \delta q_k\rangle + \frac{\Delta t}{2} \langle u(t_{k+1}), \delta q_{k+1} \rangle. 
\end{equation}
For a system with holonomic constraints specified by the manifold:
\begin{equation}
\label{eq:holonomic-cons}
    g(q) = 0 \in \mathbb{R}^m,
\end{equation}
Another action integral can be considered:
\begin{equation}
\begin{aligned}
    \int_{t_k}^{t_{k+1}} \langle \lambda(t), g(q)\rangle dt &\approx \frac{\Delta t}{2} \langle\lambda(t_k), G(q_k)\delta q_k\rangle  \\
    & + \frac{\Delta t}{2} \langle \lambda(t_{k+1}), G(q_{k+1})\delta q_{k+1}\rangle. 
\end{aligned}
\end{equation}
with \begin{equation}
\label{eq:cons-Jac}
    G(q_k) := \frac{\partial g(q_k)}{\partial q_k}
\end{equation} the Jacobian of the constraints and $\delta g(q_k) = G(q_k)\delta q_k$. 
Via adding these terms to the unconstrained Lagrangian and taking variation w.r.t $q_k$, we have the constrained dynamics:
\begin{equation}
\label{eq:dynamics-full}
\begin{aligned}
    D_1L_d(q_k, q_{k+1}) + D_2L_d(q_{k-1}, q_{k}) &= u_k\Delta t + G(q_k)^{\transpose}\lambda_k \Delta t \\
    g(q_{k+1}) &= 0
\end{aligned}.
\end{equation}
The constraints $g(q_{k+1}) = 0$ are needed to ensure the states in discrete time do not leave the manifold, which is essential in the multi-body case. 

\subsection{Discrete Null Spae Dynamics}
\tsl{Quotient space dynamics? Let me make it cooler.}\mgj{I like it. There might be existing general theorems on this.}\tsl{Yes, it exists in the literatures.}
In the case of holonomic constraints, the constrained forces are solely determined by the external force and the manifold $g(q) = 0$. Now we consider eliminating the multiplier $\lambda$ via the discrete null space method \cite{betsch2005discrete,betsch2006discrete,leyendecker2010discrete} to reduce the variables needed to determine the motion of the systems. 

Consider the constraints \eqref{eq:holonomic-cons} and its Jacobian \eqref{eq:cons-Jac}. Assume that the constraints $g(q_k) \in\mathrm{} $ is not degenerate such that
\begin{equation}
    \operatorname{Rank}(G(q)) = \dim g(q) = m,
\end{equation}
we can define the null space of $G(q)$ as the column space of $G_{\perp}(q) \in \mathrm{R}^{n\times (n - m) } $, such that:
\begin{equation}
    G_{\perp}(q) := [G_{\perp, 1}(q), G_{\perp, 2}(q), \cdots, G_{\perp, n-m}(q)],
\end{equation}
with $G_{\perp, 1}\in \mathbb{R}^{n\times 1}$, and 
\begin{equation}
    G(q) G_{\perp, i}(q) = 0, \forall i = 1, 2, \cdots, n-m.
\end{equation}
Thus, we have:
\begin{equation}
\label{eq:null-space-G}
    G^{\transpose}_{\perp}(q)G(q)^{\transpose} = 0 \Rightarrow G^{\transpose}_{\perp}(q_k)G(q_k)^{\transpose}\lambda_k = 0.
\end{equation}
Via integrating the \eqref{eq:null-space-G} to \eqref{eq:dynamics-full}, the constrained dynamics becomes: % , we have: \begin{equation} G^{\transpose}_{\perp}(q_k)G(q_k)^{\transpose}\lambda_k = 0, \end{equation}
\begin{equation}
\label{eq:dynamics-reduced}
\begin{aligned}
    G^{\transpose}_{\perp}(q_k)(D_1L_d(q_k, q_{k+1}) + D_2L_d(q_{k-1}, q_{k})) &= G^{\transpose}_{\perp}(q_k)u_k\Delta t. \\
    g(q_{k+1}) &= 0.
\end{aligned}
\end{equation}
Note that the dimensions of the quotient dynamics and constraints are $n-m$ and $m$, respectively. As the sum equals the DOF of the systems $n$, the state can be locally uniquely determined by \eqref{eq:dynamics-reduced}. Though the null space $G_{\perp}(q)$ in generalized coordinates can hardly be obtained other than numerical matrix decomposition, we note that an analytical solution is possible in the matrix Lie group case. % as the constraints of mechanical parts are usually well-defined by group actions. % Cite ZX, Li's book.
% \tsl{Smith normal form to decompose $G(x)^{\transpose}$? Our argument is that there always exists such a decomposition to enable us to compute the null space analytically so we can reduce the number of variables.}

\subsection{Dynamics on $\mathrm{SO}(3)\times \mathbb{R}^3$}
Now, we derive the EoM on $\mathrm{SO}(3)\times \mathbb{R}^3$. Consider the discrete equation of motion:
\begin{equation}
\label{eq:SO3R3-kin}
\begin{aligned}
    R_{k+1} &= R_kF_k \in \mathrm{SO}(3), \\
    p_{k+1} &= p_k + v_k \Delta t,
\end{aligned}
\end{equation}
with $R_k$ the orientation, $F_k$ the discrete pose change, $p_k$ the position and $v_k$ the linear velocity, the mid-point approximation can be applied:
\begin{equation}
\label{eq:Fk_midpoint}
\begin{aligned}
    F_k := R_k^{-1}R_{k+1} \approx I + \Delta t\omega_k^{\times}, \ \ \omega_k^{\times} \approx \frac{F_k - I}{\Delta t},
\end{aligned}
\end{equation}
\begin{equation}
\label{eq:pk_midpoint}
\begin{aligned}
    \dot{p}_k = v_k \approx \frac{p_{k+1} - p_k}{\Delta t}.
\end{aligned}
\end{equation}
Thus, the kinetic and potential energy can be approximated by:
\begin{align}
    \nonumber T_d&:=\frac{1}{2\Delta t}\operatorname{tr}((F_k - I)I^b(F_k - I)^{\transpose}) + \frac{1}{2\Delta t}m\|p_{k+1} - p_k\|^2, \\
    V_d&:= m\left(\frac{p_{k+1}+p_{k}}{2}\right)^{\transpose} g \Delta t,
\end{align}
where $g \in \mathbb{R}^{3\times 1}$ is the gravity and $I^b$ the nonstandard moment of inertia \citep{marsden1999discrete} that relate the standard moment of inertia $I_b$ by $I_b = \operatorname{tr}(I^b)I_3-I^b$. Via the taking variation on $\mathrm{SO}(3) \times \mathrm{R}^3$, we have the dynamics:
\begin{equation}
\label{eq:lgvi_dynamics}
\begin{aligned}
    % &I^bF_{k+1}^{\transpose} - F_{k+1}I^b=F_k^{\transpose}I^b - I^bF_{k}, \\
    % & R_{k+1} = R_kF_k, p_{k+1} = p_k + R_kv_k\Delta t, \\
    &F_{k+1}I^b - I^bF_{k+1}^{\transpose}=I^bF_{k} - F_k^{\transpose}I^b + \tau_k^{\wedge}\Delta t^2 , \\
    &mv_{k+1} = mv_{k} + mg\Delta t + f_k\Delta t.
    % & s.t. F_k, R_k, R_{k+1}, F_{k+1}\in \mathrm{SO}(3)
\end{aligned}
\end{equation}
As the $\mathrm{SO}(3)$ is a polynomially constrained manifold, i.e, 
\begin{equation}
    \mathrm{SO}(3) := \{ R | R^{\transpose}R = I, \operatorname{det}(R) = 1 \}, 
\end{equation}
additional algebraic structure of $\mathrm{SO}(3)$ is available to simplify the constrained dynamics. 
As common mechanical constraints are defined by group actions, CITE XXX, With the additional assumption on the constraints $g(q)$ and its Jacobian $G(q)$:
\begin{assumption}[Polynomial Constraints]
\label{assumption:poly-cons}
    Consider the rigid body system defined on $q \in \mathcal{M}_{\mathrm{RB}}$ \footnote{For $\mathrm{SO}(3)$, the ambient space is $\mathbb{R}^9$}. We assume that the constraints $g(q) = 0 \in \mathbb{R}^m $ and its Jacobian $G(q) \in \mathbb{R}^{m \times n} $ are real polynomial functions. 
\end{assumption}
Then we can show the existence of the analytical decompositions of the constraints Jacobian $G(q)$:
\begin{theorem}[Existence of Analytical Quotient Dynamics]
    Under \Cref{assumption:poly-cons}, there exist $G(q)^{\perp} \in \mathbb{R}[x]^{m \times n} $ such that $G_{\perp}^{\transpose}(q)G(q) = 0$. 
\end{theorem}
\begin{proof}
\tsl{Use the module theorem over polynomial ring $\mathbb{R}[y_1, y_2, \cdots, y_n]$}    
\end{proof}

% As the translational motion is a linear motion on $\mathbb{R}^n$, we proceed to derive the second order expansion in $\mathcal{G} = \mathrm{SO}(3)$ that is non-trivial. 



% \subsection{Alternative Derivation of LGVI in Lie Algebra}
% We apply the midpoint approximation in the Lie algebra:
% \begin{equation}
%     \Delta t\xi_k = \log{(F_k)} = \log{(R^{-1}_{k+1}R_k)}.
% \end{equation}
% Then, the approximated kinetic energy takes the form:
% \begin{equation}
%     T(\xi_k) = \frac{1}{2\Delta t}\log{(R^{-1}_{k+1}R_k)}^{\transpose} J_b \log{(R^{-1}_{k+1}R_k)}.
% \end{equation}
% Let $\phi_k = \log{(R^{-1}_{k+1}R_k)}$, we have the dynamics:
% \begin{equation}
%     J(\phi_k)^{\transpose} J_b\phi_k - J(\phi_{k-1})^{\transpose} J_b\phi_{k-1} = \tau\Delta t^2,
% \end{equation}
% where the $ J(\phi_k) $ is the left Jacobian of the $\log{(\cdot)}$. \mgj{Jacobian of the log map or the group? Isn't Jacobian of the log tricky? It's a discontinuous function.} \tsl{This version is not good, I will use the matrix version. }

% \subsection{Direct Trajectory Optimization}

% \begin{problem}[Direct Trajectory Optimization of Rigid Bodies]
%     Consider the configuration space $\mathcal{M}_{RB}$ of a $N_b$ rigid body system and the set of feasible control input, the kinematics chain $f_{\mathrm{kin}}(W_k, W_{k+1}, u_k) = 0$, and dynamics $f_{\mathrm{dyn}}(W_k, W_{k+1}, u_k) = 0$ taken values in the Lie algebra, we synthesize the optimal trajectory via the optimization:
%     \begin{equation}
%         \begin{aligned}
%             \min_{ \{ X_k, W_k, u_k\} } \quad &P( X_N, W_N ) + \sum_{k=0}^{N-1} L(X_k, W_k, u_k) \\
%             \mathrm{s.t.} \quad & f_{\mathrm{kin}}(X_{k+1}, X_{k+1}, W_k) = 0 \in \mathfrak{g}, \\
%                                 & f_{\mathrm{dyn}}(W_{k+1}, W_k, u_k) = 0 \in \mathfrak{g}, \\
%                                 & g(X_{k+1}, W_{k+1}) \le 0, \\
%                                 & W_0 = W_{init}, X_0 = W_{init}, \\
%                                 & k = 0, 1, 2, \cdots, N.
%         \end{aligned}
%     \end{equation}
%     % \log{(X_{k+1}^{-1}X_kW_k)} = 0 \in \mathfrak{g}, \\
%     with $L(\cdot, \cdot, \cdot)$ the stage cost, $P(\cdot, \cdot)$ the terminal cost, $g$ the state constraints, and initial condition specified by $W_{\mathrm{init}}$ and $X_{\mathrm{init}}$.
% \end{problem}


==> text_v3/SecondOrderRigidBody-bak.tex <==
\section{Differentiate the Rigid Body Dynamics}
\label{sec:diff-srb-dynamics} % sec:srb-dynamics
In this section, we derive the first- and second-order Riemannian derivatives of kinematics and dynamics of rigid body motion. Under \Cref{assumption:Lie=Rieman}, we can apply the BCH formula of the Lie exponential to obtain the second-order retraction in \Cref{def:2nd-retraction}.

\subsection{Differentiate the Kinematic Chain}
WLOG, we consider the constraints on $\mathcal{G}$ involves a kinematic chain with finite length $n$:
\begin{equation}
\label{eq:cons_kin}
    X_1X_2\cdots X_{n-1}X_n = I \in \mathcal{G}.
\end{equation}
Thus, the vectorized constraints can be taken as:
\begin{equation}
    \log{(X_1X_2\cdots X_{n-1}X_n)} = \log{(I)}.
\end{equation}
Now we leverage the BCH formula to derive the second-order retraction at the operating point $\bar{X}_1, \bar{X}_2, \cdots, \bar{X}_n$. We denote $Y:=X_1X_2 \cdots X_N$. To avoid using Jacobians evaluated other than the identity, we first reformulated constraints \eqref{eq:cons_kin} as: % we first shift the operating point as a ``pre-conditioning''. The first step
\begin{equation}
\begin{aligned}
&Y^{-1}X_1X_2\cdots X_{n-1}X_n = Y^{-1}, \\
\Rightarrow&\log{(Y^{-1}X_1X_2\cdots X_{n-1}X_n)} = \log{(Y^{-1})}. 
\end{aligned}
\end{equation}
Consider the tangent vector $ \bar{X}_i \xi_i^{\wedge} \in \operatorname{T}_{\bar{X}_i} \mathcal{G}$, the retraction by the Riemannian exponential is:
\begin{equation}
   c_i(t) = \bar{X}_i \exp{(t\xi_i)}
\end{equation}
Note that by \Cref{assumption:Lie=Rieman}, the Lie exponential and Riemanain exponential are identical. Thus, the perturbed equation of motion along the direction of $ \xi_i $ is available and can be simplified via repeated use of adjoint action to group all the perturbations into consecutive $\exp{(\cdot)}$. Denote $X_{i, j} = X_i X_{i+1} \cdots X_j$ when $i \le j$ and $X_{i+1, i} = I$, we have the identity using the property of adjoint action:
\begin{equation}
    \begin{aligned}
    \exp{(t\xi)\bar{X}_{i,j}} % \nonumber\\
    &= \bar{X}_{i,j} (\bar{X}_{i,j}^{-1} \exp{(t\xi)} \bar{X}_{i,j}) \\ % \nonumber\\
    &= \bar{X}_{i,j} \exp{(t \operatorname{Ad}_{\bar{X}_{i, j}^{-1} } \xi)}. % \nonumber
\end{aligned}
\end{equation}
%\tsl{Whether the Riemannian exponential is compatible with the adjoint action?}
% second order retraction in \Cref{def:2nd-retraction}
The perturbed kinematic chain becomes:
\begin{equation}
\begin{aligned}
    &Y^{-1}\bar{X}_{1}\exp{(t\xi_1)}\cdots\bar{X}_{n-1}\exp{(t\xi_{n-1})} \bar{X}_{n}\exp{(t\xi_n)}\\
    % =&Y^{-1}\bar{X}_{1}\exp{(t\xi_1)} \cdots  \bar{X}_{n-1} \bar{X}_n (\bar{X}_n^{-1} \exp{(t\xi_{n-1})} \bar{X}_{n})\exp{(t\xi_n)}\\
    % &\tyl{Missing \text{bar}?}\\
    =&Y^{-1}\bar{X}_{1}\exp{(t\xi_1)} \cdots \\
    &\bar{X}_{n-1} \bar{X}_n \exp{(t \operatorname{Ad}_{\bar{X}_{n, n}^{-1} } \xi_{n-1})}\exp{(t\xi_n)}\\
     =&Y^{-1}\bar{X}_{1}\exp{(t\xi_1)} \cdots  \bar{X}_{n-2} \\
     & \bar{X}_{n-1} \bar{X}_n  (\bar{X}_{n}^{-1} \bar{X}_{n-1}^{-1} \exp{(t\xi_{n-2})} \bar{X}_{n-1} \bar{X}_n) \\
     & \exp{(t \operatorname{Ad}_{\bar{X}_{n, n}^{-1} } \xi_{n-1})}\exp{(t\xi_n)}\\
     =&Y^{-1}\bar{X}_{1}\exp{(t\xi_1)} \cdots  \bar{X}_{n-2}\bar{X}_{n-1} \bar{X}_n  \exp{(t \operatorname{Ad}_{\bar{X}_{n-1, n}^{-1} })}\\
     & \exp{(t \operatorname{Ad}_{\bar{X}_{n, n}^{-1} } \xi_{n-1})}\exp{(t\xi_n)}\\
    =&Y^{-1}\bar{X}_{1,n}\exp{(t \operatorname{Ad}_{\bar{X}_{2, n}^{-1} } \xi_{1})}\exp{(t \operatorname{Ad}_{\bar{X}_{3, n}^{-1} } \xi_{2})} \cdots \exp{(t\xi_n)} \\
    =&\exp{(t \operatorname{Ad}_{\bar{X}_{2, n}^{-1} } \xi_{1})}\exp{(t \operatorname{Ad}_{\bar{X}_{3, n}^{-1} } \xi_{2})} \cdots \exp{(t\xi_n)}.
    % & {\color{gray} TODO add some explanation, \left( = \M \phi_r(\M w_k) - \mathbb{E}[\M \phi_r(\M w_k)] \right) }
    % \\
    % =&Y^{-1}X_{1,n}\exp{(\operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i)}\exp{(\operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j)} \\
\end{aligned}
\end{equation}
% where $X_{i, j} = X_i X_{i+1} \cdots X_j$ when $i \le j$ and $X_{i+1, i} = I$. 
Then we proceed to apply the BCH formula to obtain the second-order retraction:
\begin{equation}
\begin{aligned}
     &\log{\left( \prod_{i=1}^n \exp{\left( t\operatorname{Ad}_{\bar{X}^{-1}_{i+1, n}} \xi_i \right)} \right)} \\
    =& t\operatorname{Ad}_{\bar{X}^{-1}_{2, n}} \xi_1 + \log{\left( \prod_{i=2}^n \exp{\left( t\operatorname{Ad}_{\bar{X}^{-1}_{i+1, n}} \xi_i \right)} \right)} \\
    +&  \frac{1}{2} \left[t\operatorname{Ad}_{\bar{X}^{-1}_{2, n}} \xi_1, \log{\left( \prod_{i=2}^n \exp{\left( t\operatorname{Ad}_{\bar{X}^{-1}_{i+1, n}} \xi_i \right)} \right)}\right] + \mathcal{O}(t^3)
\end{aligned}
\end{equation}
By repeated applying of BCH formula to $\log{\left( \prod_{i=k}^n \exp{\left( t\operatorname{Ad}_{\bar{X}^{-1}_{i+1, n}} \xi_i \right)} \right)}, k\ge 2$, we have the second-order retraction as: 
% \begin{equation}
% \begin{aligned}
%     &Y^{-1}X_{1,i}\exp{(\xi_i)}X_{i+1, j}\exp{(\xi_j)}X_{j+1, n} \\
%     =&Y^{-1}X_{1,i}\exp{(\xi_i)}X_{i+1, j}\exp{(\xi_j)}X_{j+1, n} \\
%     =&Y^{-1}X_{1,i}\exp{(\xi_i)}X_{i+1, n}\exp{(\operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j)} \\
%     =&Y^{-1}X_{1,n}\exp{(\operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i)}\exp{(\operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j)} \\
% \end{aligned}
% \end{equation}
\begin{equation}
     \begin{aligned}
         &\log{\left( \prod_{i=1}^n \exp{\left( t\operatorname{Ad}_{\bar{X}^{-1}_{i+1, n}} \xi_i \right)} \right)} \\
         =& t\sum_{i=1}^n \operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i + t^2\sum_{i < j} \frac{1}{2}[\operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i, \operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j] \\
         +& \mathcal{O}(t^3)
     \end{aligned}
    % \operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i + \operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j + [\operatorname{Ad}_{X_{i+1, n}^{-1}} \xi_i, \operatorname{Ad}_{X_{j+1, n}^{-1}} \xi_j] + \mathcal{O}(\|\xi\|^2)
\end{equation}
Thus, the Riemannian gradient and Hessian of the kinematic chain can be obtained by evaluating the first- and second-order terms of $t$, which only involves adjoint action without tedious computation of Jacobians of the matrix logarithmic.

\subsection{Differentiate the Dynamics and Constraints}
Consider the rotational dynamics in \eqref{eq:lgvi_dynamics}, we again use the the retraction curve along the direction $\xi^{F}_i \in \mathfrak{so}(3)$:
\begin{equation}
    c(t) = \bar{F}_i\exp{(t\xi^{F}_i)} \in SO(3). 
\end{equation}
As the \eqref{eq:lgvi_dynamics} is already a skew matrix, the vectorized perturbed dynamics can be obtained by substituting the retraction curve and applying the $(\cdot)^{\vee}$ map:
% by considering the Riemannian exponential and the vectorized via $(\cdot)^\vee$:
\begin{equation}
\begin{aligned}
    &(F_{k+1}\exp{(t\xi^{F}_{k+1})} I^b - I^b\exp{(-t\xi^{F}_{k+1})}F_{k+1}^{\transpose})^{\vee}= \\
    & \quad (I^bF_{k}\exp{(t\xi^{F}_{k})} - \exp{(-t\xi^{F}_{k})}F_k^{\transpose}I^b)^{\vee}. % + (\tau + \delta \tau_k) ^{\wedge}\Delta t^2
\end{aligned}
\end{equation}
Via the Taylor expansion of the exponential map:
\begin{equation}
    \exp{(t\xi)}\approx I + \frac{ t\xi^{\wedge} }{1!} + \frac{ t^2\xi^{\wedge2} }{2!} + \mathcal{O}(t^3),
\end{equation}
the second-order expansion can be obtained by substituting the series and keeping the first and second-order terms of $t$. % The second-order expansion of the EOM \eqref{eq:SO3R3-kin} and dynamics \eqref{eq:lgvi_dynamics} are summarized in Table. XX. 


% \subsection{Differentiate the Holonomic Constraints}
Then we apply the second-order retraction again to differentiate the holonomic constraints. Here, we consider two common constraints: pivot constraints and axis constraints. Given two rigid bodies connected by a pivot joint, we have:
\begin{equation}
    R_1r_1 + p_1 = R_2r_2 + p_2 \tag{Pivot Constraints},
\end{equation}
where $R_i$ is the orientation of the rigid body in the world frame, $p_i$ is the position of the rigid body, and $r_i$ is the position vector pointing from the center of mass (CoM) of each rigid body to the joint, represented in each rigid body frame. 
The associated second-order retraction can be computed from:
\begin{equation}
    R_1\exp{(t\xi^{R}_1)}r_1 + (p_1 + t\xi^{p}_2) = R_2\exp{(t\xi^{R}_2)}r_2 + (p_2 + t\xi^{p}_2). 
\end{equation}
To constrain the rotation to one axis, e.g, $e_z$, we have:
\begin{equation}
    \begin{aligned}
        (R_1e_{i})^{\transpose}(R_2e_z) = 0, i = x, y,
    \end{aligned} \tag{Axis Constraints}
\end{equation}
where $e_i$ is the unit vector of each axis. Then, the second-order retraction can be computed from:
\begin{equation}
    (R_1\exp{(t\xi^{R}_1)}e_{i})^{\transpose}(R_2\exp{(t\xi^{R}_2)}e_z) = 0, i = x, y,
\end{equation}
Finally, we summarize all the constraints and the corresponding second-order retraction in \Cref{table:cons_2nd_retraction}.

\begin{table*}
\centering
\caption{Summary of equations of motions for discrete rigid body dynamics and conventional constraints.}
{\renewcommand{\arraystretch}{2}
\begin{tabular}{ccc}
\hline
 & Constraints & Second-order Expansions \\ \hline
$\begin{array}{c}
    \text{Rotational} \\
    \text{Kinematics}
\end{array}$
&  $\log{Y}:=\log{( R_{k+1}^{-1}R_kF_k )} = 0 \in \mathfrak{so}(3)$   & $\begin{aligned}
% & \\
&-Y^{-1}\xi^{R}_{k+1} + F_k^{-1}\xi^R_k + \xi_k^F + \\
&0.5[-Y^{-1}\xi^R_{k+1}, F_k^{-1}\xi^R_{k} ] + 0.5[-Y^{-1}\xi^R_{k+1},\xi^F_{k} ] \\ 
&+0.5[F_k^{-1}\xi_k^R,\xi^F_{k} ] \\
% & \\
\end{aligned}$ \\ \hline
$\begin{array}{c}
    \text{Translational} \\
    \text{Kinematics}
\end{array}$  & $p_{k+1} - p_k - v_k\Delta t = 0  \in \mathbb{R}^3$ & $\xi^p_{k+1} - \xi_k^p - \xi_k^p\Delta t$ \\ \hline 
$\begin{array}{c}
    \text{Rotational} \\
    \text{Dynamics}
\end{array}$ &  $ \begin{aligned}
% & \\
    &(F_{k+1}I^b - I^bF_{k+1}^{\transpose} - (I^bF_{k} - F_k^{\transpose}I^b))^{\vee} = 0 \in \mathfrak{so}(3)
\end{aligned} $   & $\begin{aligned}
    % & \\
     &I_bF_{k+1}\xi^F_{k+1} - I_bF_k\xi^F_k \\
    +&0.5(F_{k+1}\xi_{k+1}^{F\wedge 2}I^b - I^b\xi_{k+1}^{F\wedge 2}F_{k+1}^{\transpose})^{\vee} \\
    +&0.5(I^bF_{k}\xi_{k}^{F\wedge 2} - \xi_{k}^{F\wedge 2}F_k^{\transpose}I^b)^{\vee} \\
    % & \\s
\end{aligned} $ \\ \hline
$\begin{array}{c}
    \text{Translational} \\
    \text{Dynamics}
\end{array}$  & $mv_{k+1} - mv_k - mg\Delta t = 0 \in \mathbb{R}^3$ & $m\xi^v_{k+1} - m\xi^v_k$ \\ \hline 

$\begin{array}{c}
    \text{Pivot} \\
    \text{Constraints}
\end{array}$  & $R_1r_1 + p_1 - (R_2r_2 + p_2) = 0 \in \mathbb{R}^3$ &  $\begin{aligned}
    % & \\
    &R_1(\xi^{R\wedge}_1 + 0.5\xi^{R\wedge 2}_1 )r_1 + \xi_1^{p} - \\
    & \quad R_2(\xi^{R\wedge}_2 + 0.5\xi^{R\wedge 2}_2 )r_2 + \xi_2^{p} \\
    % & \\
\end{aligned}$ \\ \hline 

$\begin{array}{c}
    % \text{Rotation} \\
    % \text{About Axis } z
    \text{Axis}\\
    \text{Constraints}
\end{array}$  & $(R_1e_{i})^{\transpose}(R_2e_z) = 0, i = x, y$ &  $\begin{aligned}
    % & \\
    -&(R_1e_{i})^{\transpose}(R_2  e_z^{\wedge})\xi_2^{R\wedge} - (R_2e_{z})^{\transpose}(R_1  e_i^{\wedge})\xi_1^{R\wedge} \\
    & \quad + 0.5(R_1e_{i})^{\transpose}(R_2 \xi_2^{R\wedge} e_z) \\
    \vspace{1pt}
    & \quad + 0.5(R_2e_{z})^{\transpose}(R_1 \xi_1^{R\wedge} e_i) \\
\end{aligned}$ \\  
\hline 
\end{tabular}}
\label{table:cons_2nd_retraction}
% }
\end{table*}

\subsection{Complexity of Differentiation}
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/max-mrb.jpg}
    \caption{Example of a rigid body system in maximal coordinates and its Jacobian. The blue block indicates the Jacobians with nonzero elements. The lighter gray box indicares zero block while the darker gray box indicate the Jacobians of the autonomous single rigid body dynamics.}
    \label{fig:max-mrb}
\end{figure*}

As the maximal coordinates formulation admits a graph structure \cite{brudigam2021integrator}, we conclude that the complexities of evaluating the first- and second-order derivatives are linear w.r.t the number of rigid bodies and kinematic pairs. The derivative for each single rigid body can be evaluated by the first four rows of \Cref{table:cons_2nd_retraction}. As the kinematic pair only involves the configuration state of two rigid body, the Hessian only involves the variable in the two rigid bodies involved. An example of the Jacobian is illustrated in \Cref{fig:max-mrb}. % Assume that the number of kinematic pairs grows no faster than linearly w.r.t, the number of rigid bodies, which is a mild assumption for kinematic chain without loop. given the list of all kinematic pairs,


% \begin{equation}
%     (R_1\bar{R}_1)^{-1}(R_2\bar{R}_2) = I \Rightarrow \log{\left( (R_1\bar{R}_1)^{-1}(R_2\bar{R}_2)\right)} = 0
% \end{equation}
% with the $\bar{R}_1$ and $\bar{R}_2$ the offset that specify the rotational axes. To differentiate the orientation constraints, we have:
% \begin{equation}
% \begin{aligned}
%     &\bar{R}^{-1}_1 \exp{(-\xi_1)} R_1^{-1}R_2\exp{(\xi_2)}\bar{R}_2 \\
% =&\bar{R}^{-1}_1 R_1^{-1}\exp{(-R_1\xi_1)}\exp{(R_2\xi_2)}R_2\bar{R}_2 \\
%    =&\bar{R}^{-1}_1 \exp{(-\xi_1)} R_1^{-1}R_2\bar{R}_2\exp{(\bar{R}^{-1}_2\xi_2)} \\
%    =&\bar{R}^{-1}_1 R_1^{-1}R_2\bar{R}_2 \exp{(- (R_1^{-1}R_2\bar{R}_2)^{-1} \xi_1)} \exp{(\bar{R}^{-1}_2\xi_2)}
% \end{aligned}
% \end{equation}
% The we shift the system to:
% \begin{equation}
%     \begin{aligned}
%         \bar{R}^{-1}_1 R_1^{-1}\exp{(-R_1\xi_1)}\exp{(R_2\xi_2)}R_2\bar{R}_2 = I \Rightarrow \\
%         \exp{(-R_1\xi_1)}\exp{(R_2\xi_2)} = ((R_1\bar{R}_1)^{-1}(R_2\bar{R}_2))^{-1}
%     \end{aligned}
% \end{equation}


% \subsection{Differentiate the Geodesic-based Cost Function}

%%
% \subsection{Discrete Rigid Body Motion}
% Now we proceed to consider the discrete rigid body motion on the matrix Lie group. Conisder the rotational motion on $\mathrm{SO}(3)$, we consider the kinematic EOM as the reconstruction:
% \begin{equation}
% \label{eq:kin_SO3}
%     R_{k+1} = R_kF_k \in \mathrm{SO}(3).
% \end{equation}
% where $R_k$ denotes the pose and $F_k$ is the pose change. The the angular velocity change can be approximated via the pose via the mid-point approximation as:
% \begin{equation}
%     \dot{\omega}^{\wedge}_k = R_{k}^{\transpose}\dot{R}_k \approx R_{k}^{\transpose}\frac{ R_{k+1} - R_k }{\Delta t} = \frac{ F_k - I }{\Delta t}.
% \end{equation}
% Given the approximation, we have the approximated Lagrangian
% \begin{equation}
%     L(R_k, R_{k+1}) = L(F_k) = \frac{1}{2}\operatorname{tr}( \frac{ (F_k - I) }{\Delta t} J_d \frac{ (F_k - I) }{\Delta t} )\Delta t.
% \end{equation}
% thus, we have the equation of motion as: 
% \begin{equation}
% \label{eq:dyn_SO3}
% \begin{aligned}
%     % R_{k+1} &= R_kF_k \\
%     F_{k+1}J_d - J_dF^{\transpose}_{k+1} = J_dF_k - F_k^{\transpose}J_d
% \end{aligned}
% \end{equation}
% % By the definition of the non-standard inertial, we have:
% % \begin{equation}
% %     (J\omega)^{\wedge} = \omega^{\wedge}J_d + J_d\omega^{\wedge}. 
% % \end{equation}
% We have the standard inertia $J_b$ relates to the non-standard inertia $J_d$ following:
% \begin{equation}
%     J_b = \tr(J_d)I - J_d.
% \end{equation}

% Consider translational motion in the world frame we have the velocity in the world frame as:
% \begin{equation}
%     v_k = \frac{p_{k+1} - p_{k}}{\Delta t}
% \end{equation}
% Thus we have the kinetic and potential energy as:
% \begin{equation}
%     T(v) = \frac{\Delta t}{2}m(\frac{p_{k+1} - p_{k}}{\Delta t})^2. 
% \end{equation}
% and 
% \begin{equation}
%     V = mg\frac{p_{k+1} + p_k}{2}\Delta t. 
% \end{equation}
% Thus we have the EoM as:
% \begin{equation}
% \label{eq:kin_R3}
%     p_{k+1} = p_k + v_k \Delta t,  \\
% \end{equation}
% \begin{equation}
% \label{eq:dyn_R3}
%     mv_{k+1} = mv_k + mg\Delta t.
% \end{equation}
% To sum up, for a single rigid body defined on $\mathrm{SO}(3) \times \mathbb{R}^3$, we have the rigid body motion \eqref{eq:kin_SO3}, \eqref{eq:dyn_SO3}, \eqref{eq:kin_R3} and \eqref{eq:dyn_R3}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SRB on matrix Lie group %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Discrete Rigid Body Motion}
% \tsl{Review the definition of inertia tensor for general matrix Lie group. Each point is associated with a mass and velocity. }
% We first introduce the inertia tensor defined on the matrix. Consider the kinetic energy, we have the velocity on certain point of the robot:
% \begin{equation}
%     v = \xi^{\wedge} \rho,
% \end{equation}
% with $\rho$ a vector. Thus, we have the kinetic energy:
% \begin{equation}
% \begin{aligned}
%     K &= \int_{\mathcal{K}} \frac{1}{2}\| \xi^{\wedge}\rho \|^2 dm \\
%       &= \int_{\mathcal{K}} \frac{1}{2} \operatorname{tr}( \rho^{\transpose}\xi^{\wedge}\xi^{\wedge}\rho )  dm \\
%       &= \int_{\mathcal{K}} \frac{1}{2} \operatorname{tr}( \xi^{\wedge}\rho\rho^{\transpose}\xi^{\wedge} )  dm \\
%       &=  \frac{1}{2} \operatorname{tr}( \xi^{\wedge}\int_{\mathcal{K}}(\rho\rho^{\transpose})\xi^{\wedge} )  dm \\
%       &=  \frac{1}{2} \operatorname{tr}( \xi^{\wedge} J_d\xi^{\wedge} ) \\
% \end{aligned}
% \end{equation}
% and the non-standard inertia associated to the Lie algebra.
% Now we proceed to consider the discrete rigid body motion on the matrix Lie group $\mathcal{G}$, we consider the discrete kinematic as:
% \begin{equation}
% \label{eq:kin_SO3}
%     X_{k+1} = X_kW_k \in \mathcal{G}.
% \end{equation}
% where $X_k$ denotes the pose and $W_k$ is the pose change. The angular velocity change can be approximated via the pose via the mid-point approximation as:
% \begin{equation}
%     \dot{\xi}^{\wedge}_k = X_{k}^{-1}\dot{X}_k \approx X_{k}^{-1}\frac{ X_{k+1} - X_k }{\Delta t} = \frac{W_k - I }{\Delta t}.
% \end{equation}
% Given the approximation, we have the approximated Lagrangian:
% \begin{equation}
%     L(X_k, X_{k+1}) = L(W_k) = \frac{\Delta t}{2}\operatorname{tr}{\left( (\frac{W_k - I }{\Delta t}) J_d (\frac{ W_k - I }{\Delta t})^{\transpose} \right)}.
% \end{equation}
% Consider the perturbation $X_k\exp{(t\xi_k)}$ we have: 
% \tsl{Does the perturbation need to be Riemannian or the Lie exponential? Does the variation depend on metric? }
% \begin{equation}
% \begin{aligned}
%      &L(X_k\exp{(t\xi_k)}, X_{k+1}\exp{(t\xi_{k+1})}) \\
%     % =&\frac{1}{2\Delta t}\operatorname{tr}{\left( ({\exp{(-t\xi_{k})}W_k\exp{(t\xi_{k+1})} - I }) J_d (\exp{(-t\xi_{k})}W_k\exp{(t\xi_{k+1})} - I)^{\transpose} \right)}
%     =&\frac{1}{2\Delta t}\|\exp{(-t\xi_{k})}W_k\exp{(t\xi_{k+1})} - I \|^2_{J_d}
% \end{aligned}
% \end{equation}
% Via \eqref{eq:discrete_eom}, we have:
% \begin{equation}
%     \langle W_k - I, \xi_{k}^{\wedge}W_k  \rangle_{J_d} + \langle W_{k-1} - I, W_{k-1}\xi_{k}^{\wedge}  \rangle_{J_d} = 0
% \end{equation}
% with the inner product is induced by the trace function, with:
% \begin{equation}
%     \langle X, Y \rangle_P := \operatorname{tr}(XPY^{\transpose}).
% \end{equation}
% For group $\mathcal{G}$, we need to leverage the specific property of the associated property of its Lie algebra to obtain the dynamics. WLOG, we assume that the dynamics take the form:
% \begin{equation}
%     f(W_k ,W_{k+1}) = 0.
% \end{equation}
% % thus, we have the equation of motion as: 
% % \begin{equation}
% % \label{eq:dyn_SO3}
% % \begin{aligned}
% %     % R_{k+1} &= R_kF_k \\
% %     W_{k+1}J_d - J_dW^{\transpose}_{k+1} = J_dW_k - W_k^{\transpose}J_d
% % \end{aligned}
% % \end{equation}


% % By the definition of the non-standard inertial, we have:
% % \begin{equation}
% %     (J\omega)^{\wedge} = \omega^{\wedge}J_d + J_d\omega^{\wedge}. 
% % \end{equation}
% % We have the standard inertia $J_b$ relates to the non-standard inertia $J_d$ following:
% % \begin{equation}
% %     J_b = \tr(J_d)I - J_d.
% % \end{equation}

% % Consider translational motion in the world frame we have the velocity in the world frame as:
% % \begin{equation}
% %     v_k = \frac{p_{k+1} - p_{k}}{\Delta t}
% % \end{equation}
% % Thus we have the kinetic and potential energy as:
% % \begin{equation}
% %     T(v) = \frac{\Delta t}{2}m(\frac{p_{k+1} - p_{k}}{\Delta t})^2. 
% % \end{equation}
% % and 
% % \begin{equation}
% %     V = mg\frac{p_{k+1} + p_k}{2}\Delta t. 
% % \end{equation}
% % Thus we have the EoM as:
% % \begin{equation}
% % \label{eq:kin_R3}
% %     p_{k+1} = p_k + v_k \Delta t,  \\
% % \end{equation}
% % \begin{equation}
% % \label{eq:dyn_R3}
% %     mv_{k+1} = mv_k + mg\Delta t.
% % \end{equation}
% % To sum up, for a single rigid body defined on $\mathrm{SO}(3) \times \mathbb{R}^3$, we have the rigid body motion \eqref{eq:kin_SO3}, \eqref{eq:dyn_SO3}, \eqref{eq:kin_R3} and \eqref{eq:dyn_R3}.

% % \subsection{Riemmanina Metric on Matrix Lie Group}
% % In this work, we consider the canonical left-invariant metric as


% \subsection{Canonical Riemannian Connection on $\mathrm{SO}(3)$ }
% % The key to obtain the first and second-order is to leverage property of Lie exponential map  
% We use second-order retraction in \Cref{def:2nd-retraction} to obtain the Hessian and gradients of the constraints. Before we obtain the derivative, we have to define the retraction curve. Ideally, we choose the retraction curve as the Riemannian exponential map that has zero accelerations along the curve. In $\mathrm{SO}(3)$, we consider the inner product induced by the killing form as the bi-invariant metric. In this case, we have the Riemannian exponential identical to the Lie exponential. Consider the canonical basis $\left\{e_x, e_y, e_z\right\}$ as
% \begin{equation}
% \begin{aligned}
% &e_x=\left[\begin{array}{rrr}
% 0 & 0 & 0 \\
% 0 & 0 & -1 \\
% 0 & 1 & 0
% \end{array}\right], e_y=\left[\begin{array}{rrr}
% 0 & 0 & 1 \\
% 0 & 0 & 0 \\
% -1 & 0 & 0
% \end{array}\right],  \\
% &e_z=\left[\begin{array}{rrr}
% 0 & -1 & 0 \\
% 1 & 0 & 0 \\
% 0 & 0 & 0
% \end{array}\right] .
% \end{aligned}
% \end{equation}
% and their corresponding bi-invariant vector field $\left\{E_x, E_y, E_z\right\}$, we have the Riemannian connection:
% \begin{equation}
% \begin{aligned}
% \nabla_{E_x} E_y & =\frac{1}{2} E_z, & \nabla_{E_x} E_z & =-\frac{1}{2} E_y, \\
% \nabla_{E_y} E_z & =\frac{1}{2} E_x, & \nabla_{E_y} E_x & =-\frac{1}{2} E_z, \\
% \nabla_{E_z} E_x & =\frac{1}{2} E_y, & \nabla_{E_z} E_y & =-\frac{1}{2} E_x .
% \end{aligned}
% \end{equation}
% where all the other terms equal to $0$.

